Convergence Laws for Extensions of First-Order Logic with Averaging

For many standard models of random structure, first-order logic sentences exhibit a convergence phenomenon on random inputs. The most well-known example is for random graphs with constant edge probability, where the probabilities of first-order sentences converge to 0 or 1. In other cases, such as certain ``sparse random graph'' models, the probabilities of sentences converge, although not necessarily to 0 or 1. In this work we deal with extensions of first-order logic with aggregate operators, variations of averaging. These logics will consist of real-valued terms, and we allow arbitrary Lipschitz functions to be used as ``connectives''. We show that some of the well-known convergence laws extend to this setting.

==> linearsparseauxiliaryresults.tex <==
\subsection{Auxiliary results about controllers and games} \label{subsec:aux}



\begin{obs}
\label{obs:core_aux}
    Let $\GG$, $\HH$ be MRFGs and $r\geq r^\prime \geq 0$ be integers. The following facts hold:
    \begin{itemize}
        \item $\coreof{\GG \sqcup \HH}{r} = \coreof{\GG}{r} \sqcup \coreof{\HH}{r}$.
        \item $(\GG\vert_r)\vert_{r^\prime} = \GG\vert_{r^\prime}$.
        \item Let $v\in V(G)$ be such that $\ball_{r^\prime}(v) \subseteq \GG\vert_r[v]$. Then $(\GG\vert_r[v])\vert_{r^\prime} = 
        \GG[v]\vert_{r^\prime}$.
    \end{itemize}
\end{obs}


We now argue that a controller value only depends on its $r$-core for suitable $r$:

\begin{lemma}[Core determinacy of controllers]
\label{lem:controller_core}
Let $\tau(\bar u)\in \Aggo{\Mean, \LMean, \supl}$ be a term, and let $k=\srank(\tau) + \lmrank(\tau)$. Then, for each MRFG $\GG$ we have that:
\[
\lambda_\tau(\GG)=
\lambda_\tau(\GG\vert_{r_k}).
\]
\end{lemma}
\begin{proof}
    We prove the statement inductively on the structure of $\tau$. If $\tau$ is atomic, it clearly satisfies the statement. 
    The same is true if $\tau \equiv F(\pi_1,\dots, \pi_m)$ for some Lipschitz function $F$ and terms
    $\pi_1,\dots, \pi_m$,
    and the statement is assumed to hold for $\pi_1,\dots, \pi_m$. Suppose that $\tau(\bar u)
    \equiv \Mean_v \pi(\bar u, v)$, and $\pi$ satisfies the statement. Let $\GG$ be a 
    MRFG with $|\bar u|$ roots. Then, 
    \[
    \lambda_\tau(\GG) = \Ex_{\TT\sim \FBP}\left[ 
    \lambda_{\pi}(\GG \sqcup \TT)
    \right].
    \]
    By the induction hypothesis, 
    \[\lambda_{\pi}(\GG \sqcup \TT)=\lambda_{\pi}((\GG \sqcup \TT)\vert_{r_k}) 
    = \lambda_{\pi}(\GG\vert_{r_k} \sqcup \TT\vert_{r_k}).
    \]
    Here we have used Observation \ref{obs:core_aux} for the second equality. Now we argue that $\lambda(\GG\vert_{r_k})$ also equals this quantity. Indeed,
    \begin{align*}    
    \lambda_{\pi}(\GG\vert_{r_k} \sqcup \TT)=\lambda_{\pi}((\GG\vert_{r_k} \sqcup \TT)\vert_{r_k}) 
    &= \lambda_{\pi}((\GG\vert_{r_k})\vert_{r_k} \sqcup \TT\vert_{r_k}) \\
    &= \lambda_{\pi}(\GG\vert_{r_k} \sqcup \TT\vert_{r_k}).
    \end{align*}
    Here we have used Observation \ref{obs:core_aux} in the second and third equalities. \par
    Suppose that $\tau(\bar u) \equiv \LMean_{v E u_i} \pi(\bar u, v)$, where $\pi$ satisfies the statement, and 
    let $\GG$ be an arbitrary MRFG with $|\bar u|$ roots. Let $v\in V(G)$ be $\GG$'s $i$-th root. We have two cases. Suppose that $v$ is isolated. Then $\lambda_\tau(\GG)= \lambda_\tau(\GG\vert_{r_k})=0$. Otherwise, by induction:
    \begin{align}
    \nonumber
    \lambda_\tau(\GG) &= \frac{1}{|\Ne(v)|} \sum_{u\in \Ne(v)} \lambda_{\pi}(\GG[u])
    \\ 
    \label{eq:core_det1}
    &=\frac{1}{|\Ne(v)|} \sum_{u\in \Ne(v)} \lambda_{\pi}(\GG[u]\vert_{r_{k-1}}).
    \end{align}
    On the other hand,
    \begin{align}
    \nonumber
    \lambda_\tau(\GG\vert_{r_k})
    &= \frac{1}{|\Ne(v)|} \sum_{u\in \Ne(v)} \lambda_{\pi}(\GG\vert_{r_k}[u]) \\ 
    \label{eq:core_det2}
    &=\frac{1}{|\Ne(v)|} \sum_{u\in \Ne(v)} \lambda_{\pi}((\GG\vert_{r_k}[u])\vert_{r_{k-1}}).
    \end{align}
    Let $u\in \Ne(v)$. Using the fact that $u$ is adjacent to one of $\GG$'s roots and $r_k \geq r_{k-1} +1$ we obtain that 
    $\ball_{r_{k-1}}(u)\subseteq \GG\vert_{r_k}[u]$. Thus, by Observation \ref{obs:core_aux} $(\GG\vert_{r_k}[u]) \vert_{r_{k-1}} = (\GG[u]) \vert_{r_{k-1}}$. This proves that $\eqref{eq:core_det1}=\eqref{eq:core_det2}$, so 
    $\lambda_\tau(\GG)=\lambda_\tau(\GG\vert_{r_k})$.
    \par
    Finally, suppose that
    $\tau(\bar u)\equiv \sup_v \pi(\bar u, v)$,
    and $\pi$ satisfies the statement. Let $\GG$ be an arbitrary MRFG with $\abs{\bar u}$ roots. 
    We prove that $\lambda_\tau(\GG)\leq \lambda_\tau(\GG\vert_{r_k})$. The reverse inequality can be shown in a similar way.
    There are three cases.
    \begin{enumerate}[label=(\arabic*)]
        \item \label{item:sup on tree; lem:controller_core}
        Suppose that 
        \begin{equation}
        \label{eq:controller_core_aux1}
        \lambda_\tau(\GG)= 
            \sup_{\substack{ \TT \text{ finite rooted}\\ \text{featured tree}}} 
            \lambda_{\pi}(\GG\sqcup \TT).
        \end{equation}      
        Let $\TT$ be a finite rooted featured tree $\TT$.
        By the induction assumption:
        \[\lambda_{\pi}(\GG\sqcup \TT)
        = \lambda_{\pi}((\GG\sqcup \TT)\vert_{r_{k-1}})
        = \lambda_{\pi}((\GG\vert_{r_{k-1}} \sqcup \TT\vert_{r_{k-1}}).
        \]
        Here the second equality follows from Observation \ref{obs:core_aux}. 
        Hence, we can rewrite \eqref{eq:controller_core_aux1} as:
        \[
            \lambda_\tau(\GG)= 
            \sup_{\substack{ \TT \text{ finite rooted}\\ \text{featured tree}}} 
            \lambda_{\pi}(\GG\vert_{r_{k-1}}\sqcup \TT\vert_{r_{k-1}}).
        \]
        Arguing as in the $\Mean$ case, we obtain that
        $\lambda_{\pi}(\GG\vert_{r_k}\sqcup \TT) =
        \lambda_{\pi}((\GG\vert_{r_{k-1}} \sqcup \TT\vert_{r_{k-1}})$. 
        By the definition of $\lambda_\tau$, this implies that
        $\lambda_\tau(\GG\vert_{r_k})\geq \lambda_{\pi}((\GG\vert_{r_{k-1}} \sqcup \TT\vert_{r_{k-1}})$. Hence:
        \begin{gather*}
            \lambda_\tau(\GG) = 
            \sup_{\substack{ \TT \text{ finite rooted}\\ \text{featured tree}}} 
            \lambda_{\pi}(\GG\vert_{r_{k-1}}\sqcup \TT\vert_{r_{k-1}}) 
            \leq \lambda_\tau(\GG\vert_{r_k}),
        \end{gather*}
        as we wanted to show.
        \item Suppose that $\lambda_\tau(\GG)= \lambda_{\pi}(\GG[u])$ for some vertex $u\in V(G)$ that is at
        distance at most $2r_{k-1}$ 
        from some root of $\GG$ or some
        cycle of length at most $2r_{k-1} + 1$.
        We show that:
        \[\lambda_{\pi}(\GG[u])
        = \lambda_{\pi}(\GG\vert_{r_k}[u]) \leq
        \lambda_\tau(\GG\vert_{r_k}).
        \]
        The last inequality follows from the controller definition. We prove the first identity. By induction,
        \[
        \lambda_{\pi}(\GG[u]) =
        \lambda_{\pi}(\GG[u]\vert_{r_{k-1}}).
        \]
        Using that
        $r_k = 3r_{k-1} + 1$ we obtain  $\ball_{r_{k-1}}(u)\subseteq \GG\vert_{r_{k}}[u]$, so by Observation \ref{obs:core_aux} 
        $(\GG\vert_{r_{k}}[u])\vert_{r_{k-1}} = \GG[u]\vert_{r_{k-1}}$.
        Hence,
        \begin{align*}
        \lambda_{\pi}(\GG[u]) =
        \lambda_{\pi}(\GG[u]\vert_{r_{k-1}})
        &= \lambda_{\pi}((\GG\vert_{r_k}[u])\vert_{r_{k-1}}) \\
        &= \lambda_{\pi}(\GG\vert_{r_k}[u]),
        \end{align*}
        as we wanted to show. Here the second and third identities use the induction hypothesis.
        \item Suppose that $\lambda_\tau(\GG)= \lambda_{\pi}(\GG[u])$ for some vertex $u\in V(G)$ that is at distance greater than $2r_{k-1}$ to all roots in $\bar v$ and all cycles of length at most $2r_{k-1} + 1$. Then $\GG[u]\vert_{r_{k-1}}$ is the disjoint union of $\GG\vert_{r_{k-1}}$ and the featured rooted tree $\TT=\ball_{r_{k-1}}(u)$. This way,
        \begin{align*}
        \lambda_\tau(\GG)= \lambda_{\pi}(\GG[u]) 
        &= \lambda_{\pi}(\GG\vert_{r_{k-1}} \sqcup 
        \TT\vert_{r_{k-1}}) \\
        &= \lambda_{\pi}(\GG\sqcup\TT).
        \end{align*} 
        Hence, this is a particular case of scenario \ref{item:sup on tree; lem:controller_core} above.
    \end{enumerate}
    
\end{proof}







Before giving our model-theoretic result, we present some observations about controllers and games.

\begin{theorem}[Preservation of controllers by games]
\label{thm:controller_vs_controller_approx}
    Let $\epsilon, C>0$.
    Let $\tau(\bar u)\in \Aggo{\Mean, \LMean, \supl}$
    be a term satisfying that 
    $| \lambda_{\tau^\prime} | \leq C$ for all sub-terms $\tau^\prime$ of $\tau$, and let $k \geq \srank(\tau) + \lmrank(\tau)$ be an integer. 
    Consider two MFRGs $\GG$ and $\HH$ with $|\bar u|$ roots. Suppose that  
    $\GG \sim^\dist_{k,\epsilon,C} \HH$.
    Then 
    \begin{equation}
    \label{eq:EF_controller}
            \Big\lvert \lambda_\tau(\GG) - \lambda_\tau(\HH) \Big\rvert \leq 
    \epsilon \cdot \slope_\tau. 
    \end{equation}
\end{theorem}

\begin{proof}   
    Fix $\epsilon, C>0$. We show the result by induction on $\tau$'s structure. The statement is clearly true when $\tau$ is an atomic term. We deal with each induction step as follows: \par
     \textbf{Function application step: $\tau \equiv F(\pi_1, \dots, \pi_m)$.} Observe that
         $\srank(\pi_i)= \srank(\tau)$, and
         $\lmrank(\pi_i) = \lmrank(\tau)$ for all $i\in [m]$, so:
         \[
        \Big\lvert \lambda_{\pi_i}(\GG) - \lambda_{\pi_i}(\HH) \Big\rvert \leq 
    \epsilon \cdot \slope_{\pi_i}. 
         \]
         Hence, 
         \begin{align*}
            \Big\lvert \lambda_\tau(\GG) - \lambda_\tau(\HH) \Big\rvert 
            &\leq 
            \max_{i\in [m]} \slope_F \cdot   \Big\lvert \lambda_{\pi_i}(\GG) - \lambda_{\pi_i}(\HH) \Big\rvert \\
            &\leq
            \max_{i\in [m]} \epsilon \cdot \slope_F \cdot \slope_{\pi_i} \\
            &\leq
            \epsilon \cdot\slope_{\tau}. 
        \end{align*}
    \par
    \textbf{Global mean step: $\tau \equiv \Mean_v \pi$.} By the induction hypothesis, %in particular, 
    for any finite rooted featured tree $\TT$ it must hold that:
    \[
    \Big\lvert \lambda_{\pi}(\GG \sqcup \TT) - \lambda_{\pi}(\HH \sqcup \TT) \Big\rvert \leq 
    \epsilon \cdot \slope_{\pi}. 
    \]
    To see this, observe that $\srank(\pi) + \lmrank(\pi) \leq k$ and clearly
    $\GG\sqcup \TT \sim_{k,\epsilon,C}
    \HH\sqcup \TT $. Now 
     $\lvert \lambda_{\tau}(\GG) - \lambda_{\tau}(\HH) \rvert \leq 
    \epsilon \cdot \slope_{\tau}$ follows from the definition of $\lambda_\tau$ together with the fact that $\slope_\tau= \slope_{\pi} + 1$. \par
    \textbf{Supremum step: $\tau \equiv \sup_v \pi$.} In order to prove that the statement holds for $\tau$ it is enough to show that
    $\lambda_\tau(\GG) \leq \lambda_\tau(\HH) + \epsilon \cdot \slope_{\tau}$ 
    and 
     $\lambda_\tau(\HH) \leq \lambda_\tau(\GG) + \epsilon \cdot \slope_{\tau}$. We prove the first inequality, the second can be shown analogously. 
    There are two sub-cases corresponding to the definition of $\lambda_\tau$.
    \textbf{Sub-case 1.} Suppose there is some $v_G\in V(G)$ for which
    $\lambda_{\tau}(\GG)=
    \lambda_{\pi}(\GG[v_G])$.
    Let $v_H\in V(H)$ be a vertex
    satisfying $\GG[v_G] \sim_{k-1,\epsilon,C} 
    \HH[v_H]$. By hypothesis we have that:
        \[
    \Big\lvert \lambda_{\pi}(\GG[v_G]) - \lambda_{\pi}(\HH[v_H]) \Big\rvert \leq 
    \epsilon \cdot \slope_{\tau}, 
    \]
    using that $\slope_{\tau}=\slope_{\pi}$. Now
    $\lambda_\tau(\GG) \leq \lambda_\tau(\HH) + \epsilon \cdot \slope_{\tau}$ follows from the fact that
    $\lambda_{\pi}(\HH[v_H])\leq
    \lambda_{\tau}(\HH)$. 
    \textbf{Sub-case 2.} Suppose there is some finite featured rooted tree $\TT$ for which
    $\lambda_\tau(\GG)= \lambda_{\pi}(\GG \sqcup \TT)$. It holds that
    $\GG\sqcup \TT \sim_{k,\epsilon,C}
    \HH\sqcup \TT$. Hence, by assumption,
        \[
    \Big\lvert \lambda_{\pi}(\GG \sqcup \TT) - \lambda_{\pi}(\HH \sqcup \TT) \Big\rvert \leq 
    \epsilon \cdot \slope_{\tau}. 
    \]
    Again, now
    $\lambda_\tau(\GG) \leq \lambda_\tau(\HH) + \epsilon \cdot \slope_{\tau}$ follows from the fact that
    $\lambda_{\pi}(\HH\sqcup \TT)\leq
    \lambda_{\tau}(\HH)$. \par
    \textbf{Local mean step: $\tau \equiv \LMean_{v E u_i} \pi$.} Let $v_G, v_H$ denote the $i^{th}$ roots of $\GG$ and $\HH$ respectively. There are two cases. \textbf{Case 4.1. } Suppose that both $v_G$ and $v_H$ are isolated vertices. Then 
    $\lambda_\tau(\GG)=\lambda_\tau(\HH) = 0$, and the statement holds. \textbf{Case 4.2. } Now suppose that both $v_G$ and $v_H$ are non-isolated. Let $\Pi$ be a coupling of $\Ne(v_G)$ and $\Ne(v_H)$ satisfying \eqref{eq:coupling_game}. Then,
    \begin{align*}
        &\lvert \lambda_\tau(\GG) - \lambda_\tau(\HH) \rvert  \\ 
        &\quad= \abs*{
            \Ex_{(u_G,u_H)\sim \Pi}
            \left[  ~
            \lambda_{\pi}(\GG[u_G]) - \lambda_{\pi}(\HH[u_H]) ~
            \right]
        } \\
        &\quad\leq
        \Ex_{(u_G,u_H)\sim \Pi}\left[  
        ~ \lvert
        \lambda_{\pi}(\GG[u_G]) - \lambda_{\pi}(\HH[u_H])
        \rvert ~
        \right] \\    
        &\quad\leq
        \left(1 - \frac{\epsilon}{4C}\right) \slope_{\pi}\epsilon +
        \frac{\epsilon}{4C} 2C \\
         &\quad\leq (\slope_{\pi} + 1) \epsilon = \slope_{\tau} \epsilon.
    \end{align*}
    The first equality uses linearity of expectation, together with the fact that the marginal distributions of $u_G$ and $u_H$ are uniform over $\Ne(v_G)$ and $\Ne(v_H)$ respectively. 
    The second inequality uses the fact that
    $\GG[u_G] \sim_{k-1,\epsilon,C}\HH[u_H]$ with probability at least $1- \epsilon/4C$,
    and  $|\lambda_{\pi}|$ is bounded by $C$.\qedhere
\end{proof}





==> style.tex <==
%%%%%%%%%%%%%%%%%%%
%% LaTeX Styling %%
%%%%%%%%%%%%%%%%%%%

% Theorem styles
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{obs}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{question}[theorem]{Question}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{example}[theorem]{Example}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

% Custom paragraph sectioning
% \titleclass{\myparagraph}{straight}[\paragraph]
% \newcounter{myparagraph}
% \titleformat{\myparagraph}[runin]{\normalfont\normalsize\bfseries}{}{0em}{}[.]
% % The penultimate option below controls the vertical spacing above the paragraph
% % The last option below controls the horizontal spacing between the paragraph title and the text
% \titlespacing*{\myparagraph}{0pt}{*1}{1em}
\titleformat{\paragraph}[runin]{\normalfont\normalsize\bfseries}{}{0em}{}[.]
% The penultimate option below controls the vertical spacing above the paragraph
% The last option below controls the horizontal spacing between the paragraph title and the text
\titlespacing*{\paragraph}{0pt}{*1}{1em}
